Compromising Tor Anonymity Exploiting P2P Information Leakage

Privacy of users in P2P networks goes far beyond their current usage and is a fundamental requirement to the adoption of P2P protocols for legal usage. In a climate of cold war between these users and anti-piracy groups, more and more users are moving to anonymizing networks in an attempt to hide their identity. However, when not designed to protect users information, a P2P protocol would leak information that may compromise the identity of its users. In this paper, we first present three attacks targeting BitTorrent users on top of Tor that reveal their real IP addresses. In a second step, we analyze the Tor usage by BitTorrent users and compare it to its usage outside of Tor. Finally, we depict the risks induced by this de-anonymization and show that users' privacy violation goes beyond BitTorrent traffic and contaminates other protocols such as HTTP.

==> http_usage.tex <==
\section{Web Usage of Compromised BitTorrent Users}

\subsection{User Activity}

\begin{figure}[!t]
  \centering
  \includegraphics[height=2in]{plots/tor_http_req.eps}
  \caption{}
  \label{}
\end{figure}

\begin{figure}[!t]
  \centering
  \includegraphics[height=2in]{plots/tor_bt_http_country_histo.eps}
  \caption{Histogram of the HTTP usage per country. {\it all}
    represents the overall distribution of requests per category. The
    country codes represent the same information but for each of the
    top$20$ countries in number of requests.}
  \label{}
\end{figure}

\subsection{Semantic Specialization of Users}

